Low-Complexity Coding and Source-Optimized Clustering for Large-Scale Sensor Networks

We consider the distributed source coding problem in which correlated data picked up by scattered sensors has to be encoded separately and transmitted to a common receiver, subject to a rate-distortion constraint. Although near-tooptimal solutions based on Turbo and LDPC codes exist for this problem, in most cases the proposed techniques do not scale to networks of hundreds of sensors. We present a scalable solution based on the following key elements: (a) distortion-optimized index assignments for low-complexity distributed quantization, (b) source-optimized hierarchical clustering based on the Kullback-Leibler distance and (c) sum-product decoding on specific factor graphs exploiting the correlation of the data.

==> macro.tex <==



\newcommand{\mbf}[1]{\ensuremath{\mathbf #1} }
\newcommand{\bfK}{\mbf{K}}
\newcommand{\bfU}{\mbf{U}}
\newcommand{\bfu}{\mbf{u}}
\newcommand{\Uest}{\ensuremath{\hat{\bfu}}}
\newcommand{\bfI}{\mbf{I}}
\newcommand{\bfi}{\mbf{i}}
\newcommand{\bfY}{\mbf{y}}
\newcommand{\bfx}{\mbf{x}}

\newcommand{\bfR}{\mbf{R}}
\newcommand{\bfa}{\mbf{a}}
\newcommand{\bfb}{\mbf{b}}
\newcommand{\bfd}{\mbf{d}}
\newcommand{\bfc}{\mbf{c}}
\newcommand{\bfz}{\mbf{z}}
\newcommand{\levels}{\ensuremath{\mathcal L}}
\newcommand{\refeqn}[1]{(\ref{#1})}


\DeclareOldFontCommand{\rm}{\normalfont\rmfamily}{\mathrm}
\DeclareOldFontCommand{\sf}{\normalfont\sffamily}{\mathsf}
\DeclareOldFontCommand{\tt}{\normalfont\ttfamily}{\mathtt}
\DeclareOldFontCommand{\bf}{\normalfont\bfseries}{\mathbf}
\DeclareOldFontCommand{\it}{\normalfont\itshape}{\mathit}
\DeclareOldFontCommand{\sl}{\normalfont\slshape}{\@nomath\sl}
\DeclareOldFontCommand{\sc}{\normalfont\scshape}{\@nomath\sc}

%\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
%\newtheorem{definition}{Definition}

%\newcommand{\ignore}[1]{}
\newcommand{\sm}{\small}
\newcommand{\smi}{\small\it}
\newcommand{\fs}{\footnotesize}
\newcommand{\fsi}{\footnotesize\it}
\newcommand{\dsr}{\displaystyle\rm}
\newcommand{\tsr}{\textstyle\rm}
\newcommand{\ssr}{\scriptstyle\rm}
\newcommand{\sssr}{\scriptscriptstyle\rm}
\newcommand{\comment}[1]{}
\newcommand{\bfrm}[1]{\mbox{\bf#1}}
\newcommand{\bm}{\boldmath}
\newcommand{\ubm}{\unboldmath}
\newcommand{\bfit}[1]{\mbox{\boldmath$#1$}}
\newcommand{\straight}[1]{\mbox{\rm#1}}
\newcommand{\st}{\straight}
\newcommand{\jm}{\jmath\, }
%\newcommand{\correspond}{\mbox{$\hspace{.1cm}\circ\hspace{-0.4mm}\rule[0.9mm]{.5cm}%
%{0.2mm}\hspace{-1.2mm}\bullet$\hspace{0.1cm}}}
%\newcommand{\invcorrespond}{\mbox{$\hspace{.1cm}\bullet\hspace{-1.2mm}\rule[0.9mm]%
%{.5cm}{0.2mm}\hspace{-0.4mm}\circ\hspace{0.1cm$}}}
%\newcommand{\vertcorrespond}{\parbox{0.5cm}{$\circ$\hspace*{-1.12mm}$\rule[-.6cm]{0.2mm}{.6cm}$
%\par \vspace*{-.05cm}$\bullet$}}
%\newcommand{\invvertcorrespond}{\parbox{0.5cm}{$\bullet$\hspace*{-1.12mm}$\rule[-.5cm]{0.2mm}{.6cm}$
%\par \vspace*{-.05cm}$\circ$}}
%
%%\newcommand{\horizcorrespond}{\mbox{\raisebox{0.43cm}{$\circ$}\hspace{-0.14cm}%
%%\rule{0.2mm}{.5cm}\hspace{-0.1cm}\raisebox{-0.2cm}{$\bullet$}}}
%\newcommand{\si}[1]{\frac{\sin\left(#1\right)}{#1}}
%\newcommand{\sifunc}[1]{{\rm si}\left(#1\right)}
%\newcommand{\intl}{\int\limits}
%\newcommand{\intnl}{\int\nolimits}
%\newcommand{\prodl}{\prod\limits}
%\newcommand{\prodnl}{\prod\nolimits}
%\newcommand{\suml}{\sum\limits}
%\newcommand{\sumnl}{\sum\nolimits}
%\newcommand{\Real}[1]{\st{Re}\left\{#1\right\}}
%\newcommand{\Imag}[1]{\st{Im}\left\{#1\right\}}
%\newcommand{\op}[2]{\st{#1}\left\{#2\right\}}
%\newcommand{\vphi}{\varphi}
%\newcommand{\dB}{\mbox{d\hspace{-1pt}B}}
%\newcommand{\SNR}{\mbox{S\hspace{-1pt}N\hspace{-1pt}R}}
%\newcommand{\ul}[1]{\underline{#1}}
%\newcommand{\cg}{{\mathcal N}_{\mathbb C}}
%\newcommand{\tR}{\text{R}}
%\newcommand{\rg}{{\mathcal N}_{\mathbb R}}
\newcommand{\rg}{{\mathcal N}}
%\newcommand{\tI}{\text{I}}
%\newcommand{\tE}{\text{E}}
%\newcommand{\tH}{\text{H}}
\newcommand{\tT}{\text{T}}
%\newcommand{\tL}{\text{L}}
%\newcommand{\tS}{\text{S}}
%\newcommand{\tZ}{\text{Z}}
%\newcommand{\topt}{\text{opt}}
%\newcommand{\ttot}{\text{tot}}
%\newcommand{\tid}{\,\text{d}}
%\newcommand{\tF}{\text{F}}
%\newcommand{\tFc}{\text{F}_{\text{c}}}
%\newcommand{\tFd}{\text{F}_{\text{d}}}
%\renewcommand{\Re}{\text{Re}}
%\renewcommand{\Im}{\text{Im}}
%\renewcommand{\mod}{\;\text{mod}\;}
%\newcommand{\sv}[1]{\text{\small$#1$}}
\newcommand{\fnv}[1]{\text{\footnotesize$#1$}}
%\newcommand{\tv}[1]{\text{\tiny$#1$}}
%\newcommand{\hv}[1]{\text{\huge$#1$}}
%\newcommand{\lv}[1]{\text{\large$#1$}}
%\newcommand{\Lv}[1]{\text{\Large$#1$}}
%\newcommand{\LLv}[1]{\text{\LARGE$#1$}}
\newcommand{\scomm}[1]{\quad\text{#1}\quad}
\newcommand{\comm}[1]{\qquad\text{#1}\qquad}
%\newcommand{\argmax}[1]{\underset{#1}{\text{argmax}}}
%\newcommand{\argmin}[1]{\underset{#1}{\text{argmin}}}
%\newcommand{\tm}{\footnotesize-}
%\newcommand{\tp}{\footnotesize+}
%
%
%\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Diag}{Diag}
\DeclareMathOperator{\Circ}{Circ}
\DeclareMathOperator{\ld}{ld}
%\DeclareMathOperator{\erfc}{erfc}
%\DeclareMathOperator{\Pr}{Pr}
%
%
%\newcommand{\hdt}{\operatorname{d_H}}
%\newcommand{\hwt}{\operatorname{w_H}}
%\newcommand{\atanh}{\ensuremath{\operatorname{artanh}}}
%\newcommand{\lcm}{\operatorname{lcm}}
%\newcommand{\rank}{\operatorname{rank}}
%\newcommand{\dirac}[1]{\delta(#1)}
%\newcommand{\GF}{\mathbb{F}}
%\newcommand{\scpr}[2]{\ensuremath{\langle{#1},{#2}\rangle}}
%\newcommand{\dmin}[1]{d_{min}^{\hspace*{0.5mm}#1}}
%%\newcommand{\exend}{\hfill$\Box$} % box at end of example
%\newcommand{\exend}{\hfill\ding{113}} % box at end of example
%
%\newcommand{\hlt}{\begin{align*}\hline\hspace{14cm}\end{align*}}
%\newcommand{\obw}{\textwidth-1.4cm}
%
%%
% begin equation
\newcommand{\bml}[1]{\begin{multline}\label{#1}}
\newcommand{\eml}{\end{multline}}
\newcommand{\beq}[1]{\begin{equation}\label{#1}}
\newcommand{\eeq}{\end{equation}}
% begin equation not numbered
\newcommand{\benn}{\[}
\newcommand{\eenn}{\]}
% begin eqnarray not numbered
\newcommand{\beann}{\begin{eqnarray*}}
\newcommand{\eeann}{\end{eqnarray*}}
% begin eqnarray
\newcommand{\bea}[1]{\begin{eqnarray}\label{#1}}
\newcommand{\eea}{\end{eqnarray}}
%
% begin minipage
\newcommand{\bmp}{\begin{minipage}}
\newcommand{\emp}{\end{minipage}}
\newcommand{\figspace}{\fbox{\vbox to 3cm{\parbox{11cm}{\begin{center}
Bild \end{center}}}}}
\newcommand{\equa}[1]{(\ref{#1})}
\newcommand{\bild}[1]{Figure~\ref{#1}}
\newcommand{\extra}{\vspace{.5cm}}

% 
% referencing
%
\newcommand{\eq}[1]{\eqref{#1}}
\newcommand{\fnref}[1]{footnote~\ref{#1}}
\newcommand{\liref}[1]{\ref{#1}}
\newcommand{\pg}[1]{pg.~\pageref{#1}}
\newcommand{\definref}[1]{{\itshape Definition~\ref{#1}}}
\newcommand{\theorref}[1]{{\itshape Theorem~\ref{#1}}}
\newcommand{\lemmaref}[1]{{\itshape Lemma~\ref{#1}}}
\newcommand{\corolref}[1]{{\itshape Corollary~\ref{#1}}}
\newcommand{\proporef}[1]{{\itshape Proposition~\ref{#1}}}
\newcommand{\charef}[1]{Chapter~\ref{#1}}
\newcommand{\secref}[1]{Sec.~\ref{#1}}
\newcommand{\appref}[1]{Appendix~\ref{#1}}
\newcommand{\fig}[1]{{\itshape Fig.~\ref{#1}}}
\newcommand{\figa}[2]{{\itshape Fig.~\ref{#1}(#2)}}
\newcommand{\ex}[1]{{\itshape Example~\ref{#1}}}
\newcommand{\ta}[1]{{\itshape Table~\ref{#1}}}
%
\newcommand{\chrisdef}{\stackrel{def}{=}}
\newcommand{\hdt}{\operatorname{d_H}}
\newcommand{\hwt}{\operatorname{w_H}}
\newcommand{\BC}{\mathcal{C}}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\TC}{\mathcal{C}}
\newcommand{\GF}{\mathbb{F}}
\newcommand{\vv}[1]{{\boldsymbol{#1}}}
\newcommand{\vvr}[3]{\boldsymbol{#1}_{[#2,#3)}}
\newcommand{\mm}[1]{{\boldsymbol{#1}}}
\newcommand{\sympg}[1]{{\bfseries \pageref{#1}}}
\newcommand{\dual}[1]{\ensuremath{{#1}^\perp}}
\newcommand{\convdual}[1]{\ensuremath{{#1}_\perp}}
\newcommand{\scpr}[2]{\ensuremath{\langle{#1},{#2}\rangle}}
\newcommand{\dscpr}[2]{\ensuremath{\langle{#1},{#2}\rangle_{D}}}
\newcommand{\del}[1]{\operatorname{del}(#1)}
\renewcommand{\deg}[1]{\operatorname{deg}(\ensuremath{#1})}
\newcommand{\str}[1]{#1{\hspace{-5mm}\bigg/\hspace{1mm}}}
\newcommand{\dint}{\operatorname{d}}
\newcommand{\chrismatrix}[1]{\begin{pmatrix}#1\end{pmatrix}}
\newcommand{\pboxplus}{\put(-8.0, 1.0){${\scriptstyle \boxplus}$}}
\newcommand{\poplus}{\put(-8.0, 1.0){${\scriptstyle \oplus}$}}
\renewcommand{\mod}{\operatorname{mod}}
\newcommand{\ord}{\operatorname{ord}}
\newcommand{\Bset}{\mathcal{B}}
\newcommand{\StateSp}{\Sigma}
\newcommand{\SymbolSp}{V}
\newcommand{\TrellisSection}{\mathcal{T}}
\newcommand{\Trellis}{\mathcal{T}}
\newcommand{\BranchInSection}[1]{(\vv{\sigma}_{#1},\vv{v}_{#1},\vv{\sigma}_{{#1}+1})
  \in \Bset_{#1}}
\newcommand{\BranchInDualSection}[1]{(\vv{s}_{#1},\vv{w}_{#1},\vv{s}_{{#1}+1})
  \in \dual{\Bset}_{#1}}
\newcommand{\cardinality}[1]{|#1|}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\dirac}[1]{\delta(#1)}
\newcommand{\expectation}[1]{E\{#1\}}
\newcommand{\R}{\ensuremath{{\mathcal R}}}
\newcommand{\StateSet}{\ensuremath{{\mathcal S}}}
\newcommand{\correspond}{\mbox{$\hspace{.1cm}\circ\hspace{-0.4mm}\rule[0.9mm]{.5cm}{0.2mm}\hspace{-1.2mm}\bullet$\hspace{0.1cm}}}
\newcommand{\invcorrespond}{\mbox{$\hspace{.1cm}\bullet\hspace{-1.2mm}\rule[0.9mm]{.5cm}{0.2mm}\hspace{-0.3mm}\circ$\hspace{0.1cm}}}
\newcommand{\complexn}{\ensuremath{\mathbb{C}}}
\newcommand{\Ctb}[1]{\ensuremath{{\TC}^{#1}}}
\newcommand{\Ctbdual}[1]{\ensuremath{{\TC}^{#1,\perp}}}
\newcommand{\charac}{\operatorname{\chi}}
\newcommand{\OverallSymbolSp}{\ensuremath{{\mathcal V}}}
\newcommand{\cc}[1]{\overline{#1}} % complex conjugate
\newcommand{\simfigwidth}{11cm}
\newcommand{\SM}{{\displaystyle\;\!\shortmid}}
\newcommand{\fabgr}{\ensuremath{\mathscr{A}}}
\newcommand{\CharC}{\ensuremath{\mathcal{C}}}
\newcommand{\PermMatrix}{\ensuremath{\mathcal{P}}}
\newcommand{\torus}{\ensuremath{\mathbb{T}}}
\newcommand{\Chor}{\ensuremath{{\BC}^{-}}}
\newcommand{\Cver}{\ensuremath{{\BC}^{\SM}}}
\newcommand{\blocknumberlcmlength}{J}
\newcommand{\infoblocklcm}{j}
\newcommand{\Awtenum}{A} % character used for weight enumerators
\newcommand{\Bwtenum}{B} % character used for bit weight enumerators
\newcommand{\awt}{a} % character used enumerating codewords
\newcommand{\pcbc}{{\ensuremath{\mathcal C_P}}}
\newcommand{\eventlength}{{\ensuremath{\lambda}}}
\newcommand{\Eventlength}{{\ensuremath{\Lambda}}}
\newcommand{\numberevents}{{\ensuremath{x_h}}}
\newcommand{\numbereventsone}{{\ensuremath{x_{h_1}}}}
\newcommand{\numbereventstwo}{{\ensuremath{x_{h_2}}}}
\newcommand{\numbereventsmax}{{\ensuremath{x_{h_{max}}}}}
\newcommand{\truncate}[2]{{\ensuremath{[#1]_{#2}}}}
\newcommand{\eventmultiplicity}[2]{{\ensuremath{c[#1,#2]}}}
\newcommand{\approxmultiplicity}[1]{{\ensuremath{c_{\text{TB}}[#1]}}}
\newcommand{\Constant}{\ensuremath{C}}
\newcommand{\semiringplus}{\ensuremath{\oplus}}
\newcommand{\semiringprod}{\ensuremath{\odot}}
\newcommand{\semiringplusidentity}{\textgoth{0}}
\newcommand{\semiringprodidentity}{\textgoth{1}}
\newcommand{\noisepower}{\ensuremath{N}_0}
\newcommand{\basecodelength}{\ensuremath{N}_b}
\newcommand{\baseinfolength}{\ensuremath{K}_b}
\newcommand{\constant}{\mathscr{C}}
\newcommand{\splitwef}{\ensuremath{\mathscr{S}}}
\newcommand{\lhwt}{\operatorname{w_L}}
\newcommand{\rhwt}{\operatorname{w_R}}
\newcommand{\grhwt}[1]{\operatorname{w_{R,#1}^{\ast}}}
\newcommand{\glhwt}[1]{\operatorname{w_{L,#1}^{\ast}}}
\newcommand{\gsplitwef}[2]{\ensuremath{\mathscr{S}}^{\ast}_{{#1},{#2}}}
\newcommand{\interleaver}{\ensuremath{\Pi}}
\newcommand{\dmin}[1]{d_{min}^{\hspace*{0.5mm}#1}}
\newcommand{\df}{d_{f}}
\newcommand{\dfeff}{d_{f,eff}}
\newcommand{\GolayCC}{\CC_{\mathcal{G}}}
\newcommand{\adjacencymatrix}{\ensuremath{\mm{T}}}
\newcommand{\converrorenumerator}{\ensuremath{A}}
\newcommand{\combinedTBWEF}{\ensuremath{A}}
\newcommand{\christrace}{\operatorname{tr}}
\newcommand{\convcodeclass}{\ensuremath{\mathcal{S}}}
\newcommand{\minavweight}{\ensuremath{\omega_0}}
\newcommand{\forneyindex}{\ensuremath{\nu}}
\newcommand{\thresholdforneyindex}{\ensuremath{\gamma}}
\newcommand{\embeddedcode}{\ensuremath{\mathcal{E}}}
\newcommand{\fdimension}{\ensuremath{\delta}}
\newcommand{\punct}[1]{\ensuremath{#1^{\bullet}}}
\newcommand{\ProwsofGbullet}{\ensuremath{\mm{M}}}
\newcommand{\minor}{\ensuremath{\Delta}}
\newcommand{\distspecad}{\ensuremath{a}}
\newcommand{\distspeccd}{\ensuremath{c}}
\newcommand{\dualTrellisSectionCombined}[1]{\ensuremath{\TrellisSection^{\perp}_{\text{comb},#1}}}
\newcommand{\dualTrellisCombined}{\ensuremath{\TrellisSection^{\perp}_{\text{comb}}}}
\newcommand{\combined}{\ensuremath{\text{comb}}}
\newcommand{\dualBsetCombined}[1]{\ensuremath{\Bset^{\perp}_{\text{comb},#1}}}
\newcommand{\ATB}{\ensuremath{A_{TB}}}
\newcommand{\MTB}{\ensuremath{M_{TB}}}
\newcommand{\DATB}{\ensuremath{\dual{A}_{TB}}}
\newcommand{\DMTB}{\ensuremath{\dual{M}_{TB}}}
\newcommand{\AWTB}{\ensuremath{A_{WTB}}}
\newcommand{\MWTB}{\ensuremath{M_{WTB}}}
\newcommand{\DAWTB}{\ensuremath{\dual{A}_{WTB}}}
\newcommand{\DMWTB}{\ensuremath{\dual{M}_{WTB}}}
\newcommand{\CGolayThird}{\ensuremath{\CC_{1/3}}}
\newcommand{\CGolayFourtha}{\ensuremath{\CC^a_{1/4}}}
\newcommand{\CGolayFourthb}{\ensuremath{\CC^b_{1/4}}}
\newcommand{\whiteningfilterdegree}{\ensuremath{M_f}}
\newcommand{\circlelength}{\ensuremath{l}}
\newcommand{\byteinterleaverdepth}{\ensuremath{I_{\text{RS}}}}
\newcommand{\precoderdegree}{\ensuremath{M_{\text{prec}}}}
\newcommand{\predictorpolynomialdegree}{\ensuremath{M_{\text{S}}}}
\newcommand{\predictorpolynomial}{\ensuremath{s}}
\newcommand{\prpolynomial}{\ensuremath{f_{\text{PR}}}}
\newcommand{\precoderpolynomial}{\ensuremath{p_{\text{prec}}}}
\newcommand{\codeoneappchapter}{\ensuremath{\TC_1}}
\newcommand{\codetwoappchapter}{\ensuremath{\TC_2}}
\newcommand{\codeintroturbo}{\ensuremath{\TC_F}}
\newcommand{\codeonesimresults}{\ensuremath{\TC_G}}
\newcommand{\codetwosimresults}{\ensuremath{\TC_H}}
\newcommand{\codethreesimresults}{\ensuremath{\TC_I}}
\newcommand{\Ldec}{L^{\text{dec}}}
\newcommand{\Ldecextr}{L_e^{\text{dec}}}
\newcommand{\Ldecchannel}{L_c^{\text{dec}}}
\newcommand{\Ldet}{L^{\text{det}}}
\newcommand{\Ldetapri}{L_a^{\text{det}}}
\newcommand{\writecurrent}{I_c}
% 
\def\SETN {I\hspace{-0.8ex}N}
\def\SET0N {I\hspace{-0.8ex}N_0}
\def\SETR {I\hspace{-0.8ex}R}
\def\SETZ {Z\hspace{-1.2ex}Z}
\def\SETB {I\hspace{-0.8ex}B}
\newcommand{\rend}{\hfill$\square$}
\newcommand{\tend}{\hfill$\blacksquare$}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   here we define theorem environments

%\definecolor{light}{gray}{.80}%
%\usepackage{theorem}
{%
%        \theoremstyle{plain}
%        \theoremheaderfont{\bfseries}   
%        \theorembodyfont{\sffamily}
%       \theorembodyfont{\itshape}
%        \newtheorem{example}{
%\colorbox{light}{Example}}[chapter]%
}%

{%
%        \theoremstyle{plain}
%        \theorembodyfont{\normalfont}
%        \theoremheaderfont{\normalfont}  
%%        \newtheorem{definition}{Definition}[chapter]%
%        \newtheorem{theorem}{\colorbox{light}{Theorem}}[chapter]%
%        \newtheorem{lemma}[theorem]{\colorbox{light}{Lemma}}%
%        \newtheorem{corol}[theorem]{Corollary}%
%        \newtheorem{propo}[theorem]{Proposition}%
% \newtheorem{remark}{Remark}%
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   here we define new environments
%
% enumerate with boldface letters
\newenvironment{bfenumerate}   
  {\begin{enumerate}\normalfont\bfseries}
  {\end{enumerate}}
% itemize with boldface letters
\newenvironment{bfitemize}
  {\begin{itemize}\normalfont\bfseries}
  {\end{itemize}}
% citations
\newsavebox{\Citname}
\newenvironment{Citation}[1]
 {\sbox{\Citname}{\textit{#1}}
  \begin{description}\item[\rule{15mm}{0mm}]}
  {\hspace*{\fill}\nolinebreak[1]\hspace*{\fill}%
   \usebox{\Citname}\end{description}}
% Proofs
%\newenvironment{proof}
%  {{\it Proof:} \hspace{3mm}}
%  {\par\vspace*{3mm}}
%
%\newenvironment{sketchproof}
%  {{\it Sketch of Proof:} \hspace{3mm}}
%  \tend{\par\vspace*{3mm}}
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\clearemptydoublepage}{\newpage{\pagestyle{empty}\cleardoublepage}}
% \newcommand{\longpage}{\enlargethispage{\baselineskip}}
\newcommand{\llongpage}{\enlargethispage{2cm}}
% \newcommand{\shortpage}{\enlargethispage{-\baselineskip}}
\newcommand{\ignore}[1]{}
\newcommand{\hag}[1]{#1}
\newcommand{\jD}{\displaystyle}
\newcommand{\jT}{\textstyle}
\newcommand{\jS}{\scriptstyle}
\newcommand{\jSS}{\scriptscriptstyle}
% \newcommand{\nl}{\\[2ex]} % next line with additional space
\newcommand{\nn}{\nonumber} % this line without equation number
\newcommand{\exend}{\hfill\ding{113}} % box at end of example
\newcommand{\boxend}{\hfill$\blacksquare$} % box at end of definitions,
                                           % theorems, etc.
\newcommand{\proofend}{\hfill$\blacktriangle\blacktriangle$} % box at end of proofs
\newcommand{\jenssec}[2]{\ensuremath{{#1}_0,{#1}_1,\dotsc,{#1}_{#2}}}
\newcommand{\jensmod}[1]{\ensuremath{\bmod{#1}}}
\newcommand{\cond}{\,|\,}
\newcommand{\conda}{\,\rule{0.5pt}{7pt}\,}
\newcommand{\isom}{\simeq}
\newcommand{\cctr}{\dagger} %  transpose matrix and make entries conjugate
                            %  complex
\newcommand{\pzp}[1]{\overline{#1}} % product of polynomials in Z_p
\newcommand{\ft}[1]{{#1}^{\star}} % Fourier transform
\newcommand{\ift}[1]{\overleftarrow{#1}} % inverse Fourier transform
\newcommand{\fcorr}{\mbox{$\hspace{.1cm}\circ\hspace{-0.4mm}\rule[0.9mm]{.5cm}{0.2mm}\hspace{-1.2mm}\bullet$\hspace{0.1cm}}}
\newcommand{\invfcorr}{\mbox{$\hspace{.1cm}\bullet\hspace{-1.2mm}\rule[0.9mm]{.5cm}{0.2mm}\hspace{-0.3mm}\circ$\hspace{0.1cm}}}
\newcommand{\fcor}{\mbox{$\circ\hspace{-0.4mm}\rule[0.9mm]{.5cm}{0.2mm}\hspace{-1.2mm}\bullet$}}
\newcommand{\invfcor}{\mbox{$\bullet\hspace{-1.2mm}\rule[0.9mm]{.5cm}{0.2mm}\hspace{-0.3mm}\circ$}}
\newcommand{\concat}[1]{\underset{#1}{\land}}
\newcommand{\jensfor}{\quad\text{for}\quad}
\newcommand{\suml}{\sum\limits}
\newcommand{\intl}{\int\limits}
\newcommand{\prodl}{\prod\limits}
\newcommand{\bs}[1]{{\boldsymbol{#1}}}
\newcommand{\expect}[1]{\ensuremath{\operatorname{E}\left[#1\right]}}
\newcommand{\variance}[1]{\ensuremath{\operatorname{Var}\left[#1\right]}}
\newcommand{\cwt}{\operatorname{v}}% composition weight function
\newcommand{\wt}{\operatorname{w}}

\newcommand{\edt}{\operatorname{d_E^2}}
\newcommand{\ewt}{\operatorname{w_E^2}}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\ind}{\operatorname{ind}}
\newcommand{\bessel}{\ensuremath{\operatorname{I_0}}}
\newcommand{\atanh}{\ensuremath{\operatorname{artanh}}}
\newcommand{\erfc}{\ensuremath{\operatorname{erfc}}}
\newcommand{\dB}{~\mathrm{dB}}
\newcommand{\lcm}{\operatorname{lcm}}
\newcommand{\kernel}{\operatorname{Ker}}
\newcommand{\image}{\operatorname{Im}}
\newcommand{\comp}{\operatorname{comp}} % composition of a sequence
\newcommand{\scpro}[2]{\ensuremath{\langle\langle{#1},{#2}\rangle\rangle}}
\newcommand{\scprd}[2]{\ensuremath{\langle{#1},{#2}\rangle_{D}}}
\newcommand{\trace}[2]{\ensuremath{\operatorname{Tr}_{#1}\left(#2\right)}}
\newcommand{\tracef}[1]{\ensuremath{\operatorname{Tr}_{#1}}}
% 
\newcommand{\ie}{i.e.}
\newcommand{\cf}{cf.~}
\newcommand{\eg}{e.g.~}
\newcommand{\Eg}{E.g.~}
\newcommand{\etal}{et~al.}
\newcommand{\viz}{viz.~}
\newcommand{\etc}{etc.}
\newcommand{\foin}{for instance~}
\newcommand{\akz}[1]{``#1''} % Gaensefuesschen
\newcommand{\apri}{\emph{a priori}~}
\newcommand{\apost}{\emph{a posteriori}~}
\newcommand{\GFq}{\ensuremath{\GF{q}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\Zq}{\ensuremath{\Z_q}}
\newcommand{\jenscal}[1]{\ensuremath{{\mathcal #1}}}
\newcommand{\F}{\ensuremath{{\mathcal F}}}
\newcommand{\G}{\ensuremath{{\mathcal G}}}
\newcommand{\A}{\ensuremath{{\mathcal A}}}
\newcommand{\HH}{\ensuremath{{\mathcal H}}}
\newcommand{\module}{\ensuremath{{\mathcal M}}}
\newcommand{\group}[1]{\ensuremath{{\mathcal #1}}} 
\newcommand{\ra}{\to}
\newcommand{\da}{\downarrow}


